Put Teacher in Student's Shoes: Cross-Distillation for Ultra-compact Model Compression Framework

In the era of mobile computing, deploying efficient Natural Language Processing (NLP) models in resource-restricted edge settings presents significant challenges, particularly in environments requiring strict privacy compliance, real-time responsiveness, and diverse multi-tasking capabilities. These challenges create a fundamental need for ultra-compact models that maintain strong performance across various NLP tasks while adhering to stringent memory constraints. To this end, we introduce Edge ultra-lIte BERT framework (EI-BERT) with a novel cross-distillation method. EI-BERT efficiently compresses models through a comprehensive pipeline including hard token pruning, cross-distillation and parameter quantization. Specifically, the cross-distillation method uniquely positions the teacher model to understand the student model's perspective, ensuring efficient knowledge transfer through parameter integration and the mutual interplay between models. Through extensive experiments, we achieve a remarkably compact BERT-based model of only 1.91 MB - the smallest to date for Natural Language Understanding (NLU) tasks. This ultra-compact model has been successfully deployed across multiple scenarios within the Alipay ecosystem, demonstrating significant improvements in real-world applications. For example, it has been integrated into Alipay's live Edge Recommendation system since January 2024, currently serving the app's recommendation traffic across \textbf{8.4 million daily active devices}.

==> Content/Table/TableDeployment.tex <==

\begin{table}[]
\caption{Time Cost of EI-BERT Framework}
\vspace{-5pt}
\label{tab:deploymnet}
\begin{tabular}{l|cc|c}
\hline
Platform & \multicolumn{1}{l}{ Inference~(ms)} & \multicolumn{1}{l|}{{Compilation~(ms) }} & \multicolumn{1}{l}{overall} \\ \hline
Andriod  & 45.17                                  & 103.78                                                           & 148.95                      \\
iOS      & 39.29                                  & 60.27                                                            & 99.56                       \\ \hline
\end{tabular}
\vspace{-15pt}
\end{table}
